SODA: Protecting Proprietary Information in On-Device Machine Learning Models

The growth of low-end hardware has led to a proliferation of machine learning-based services in edge applications. These applications gather contextual information about users and provide some services, such as personalized offers, through a machine learning (ML) model. A growing practice has been to deploy such ML models on the user's device to reduce latency, maintain user privacy, and minimize continuous reliance on a centralized source. However, deploying ML models on the user's edge device can leak proprietary information about the service provider. In this work, we investigate on-device ML models that are used to provide mobile services and demonstrate how simple attacks can leak proprietary information of the service provider. We show that different adversaries can easily exploit such models to maximize their profit and accomplish content theft. Motivated by the need to thwart such attacks, we present an end-to-end framework, SODA, for deploying and serving on edge devices while defending against adversarial usage. Our results demonstrate that SODA can detect adversarial usage with 89% accuracy in less than 50 queries with minimal impact on service performance, latency, and storage.

==> archive/buffer.tex <==
\section{Introduction}
Consider the following motivating examples.

\begin{enumerate}
    \item \textbf{Credit card offers:} Consider a bank application which produces personalized credit card offers based on users’ contextual information. Assume a ML model is deployed to do this. Here the distribution and range of offers available along with who is recommended what is proprietary information. An adversary can learn what sets of inputs give them the most profitable output by learning the probability distribution of the potential offers. 
    
    \item \textbf{Image authentication:} Consider an image authentication service which accepts or rejects images onto a social media platform based on their authenticity. Here the criteria or rules embedded in the model are proprietary information. An adversary can learn the rules by investigating the model's most salient features and distort the input in minor ways to authenticate disallowed images.

    \item \textbf{Life insurance risk assessment:} Consider a life insurance risk assessment model that determines the level of insurance risk for users. Here the hidden representation, or how the risk assessment is done, is proprietary information. An adversary can learn the correlations between attributes and differing risk levels to gouge what an insurance company finds more or less risk inducing, and try to hack the input in ways beneficial to them.

    \item \textbf{Health assessment: } Consider a mobile application which collects sensitive health information to provide medical assessments (e.g., diagnoses and treatments). Here the representations mapping health information to assessments is proprietary information. An adversary can learn the representations and misuse the information for self assessments or detect biases.
\end{enumerate}


\section{Preserving Proprietary Information in 
On-Device Models}

Deploying models on device reduces the service provider’s authority of its usage and makes it difficult to track or identify adversarial actions. In this section, we propose an end-to-end modeling system for deploying and serving ML models on device while protecting the proprietary information embedded in the model using protection and defense layers. We then evaluate the efficacy of the proposed system.

\subsection{System Design}
The system design is two-fold with protection and defense embedded into the application pipeline as demonstrated in Figure \ref{}. The protection layer involves random-weighted serving using an ensemble model and the defense layer involves an adversarial usage detector which labels consequent queries as benign, suspicious and adversarial. We describe these two components of the system in further details as follows. 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/example_tree1.png}
    \caption{}
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/example_tree2.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/example_tree3.png}
    \caption{}
    \end{subfigure}
    \\
    %
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/rf.png}
    \caption{}
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/rf_weighted_w[0.3, 0.6, 0.1].png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/rf_weighted_w[0.1, 0.3, 0.6].png}
    \caption{}
    \end{subfigure}
    %
    \caption{Intuitive example of random weighted averaging on a random forest (RF) with three trees trained on a toy binary classification problem with two features. (a)-(c) show the decision boundaries of each tree in the ensemble. (d) shows the decision boundary of the random forest when aggregated using traditional methods (e.g., averaging). (e)-(f) show decision boundaries of randomly weighting each tree during aggregation.}
    \label{fig:ensemble_intuition}
\end{figure*}

\subsubsection{Protecting}
A single model is more susceptible to attacks due to lack of its robustness and generalization abilities making it easier to exploit via out-of-distribution queries. We propose to an ensemble model that serves using random weighted averaging. This causes the decision boundaries to widen in a randomized manner, removing variance and improving generalization. For example, Figure \ref{fig:ensemble_intuition} demonstrates...Intuitively, this protects against the first group of attacks which exploit the lack of robustness in ML models.

TODO: describe sampling process, training process and serving process

\subsubsection{Defending}
Due to the offline component of on-device models, an adversary with unlimited resources can still exploit an ensemble model outside the knowledge of the service provider. To thwart this problem, we build an adversarial detector that identifies adversarial usage across time and blocks the user from making further queries to the model. This detector extracts features pertaining to query rates, query distributions, and leakage to classify usage type into benign, suspicious or adversarial. The defense is meant to target adversaries with varying prior knowledge.

Intuition: prior defenses make assumptions on the nature of the queries including what distribution they follow and whether they are in distribution or out of distribution. As we see in Figure \ref{fig:intuition-distribution}, random querying attacks may still follow a normal distribution but the distance between the queries changes substantially.

\subsection{System Evaluation}

% aatrey@swarm:~/work1/private-ondevice-ml$ hostnamectl
%    Static hostname: swarm
%          Icon name: computer-server
%            Chassis: server
%         Machine ID: 690284d4dcc347fe88793d68c3fc4a7c
%            Boot ID: 1e72be1c0aef4f098c35cc07372492de
%   Operating System: Ubuntu 20.04.4 LTS
%             Kernel: Linux 5.4.0-131-generic
%       Architecture: x86-64

% aatrey@swarm:~/work1/private-ondevice-ml$ lscpu
% Architecture:                    x86_64
% CPU op-mode(s):                  32-bit, 64-bit
% Byte Order:                      Little Endian
% Address sizes:                   46 bits physical, 48 bits virtual
% CPU(s):                          48
% On-line CPU(s) list:             0-47
% Thread(s) per core:              2
% Core(s) per socket:              12
% Socket(s):                       2
% NUMA node(s):                    2
% Vendor ID:                       GenuineIntel
% CPU family:                      6
% Model:                           79
% Model name:                      Intel(R) Xeon(R) CPU E5-2650 v4 @ 2.20GHz
% Stepping:                        1
% CPU MHz:                         1200.512
% CPU max MHz:                     2900.0000
% CPU min MHz:                     1200.0000
% BogoMIPS:                        4400.42
% Virtualization:                  VT-x
% L1d cache:                       768 KiB
% L1i cache:                       768 KiB
% L2 cache:                        6 MiB
% L3 cache:                        60 MiB


